Temporal Attention Model for Neural Machine Translation

Attention-based Neural Machine Translation (NMT) models suffer from attention deficiency issues as has been observed in recent research. We propose a novel mechanism to address some of these limitations and improve the NMT attention. Specifically, our approach memorizes the alignments temporally (within each sentence) and modulates the attention with the accumulated temporal memory, as the decoder generates the candidate translation. We compare our approach against the baseline NMT model and two other related approaches that address this issue either explicitly or implicitly. Large-scale experiments on two language pairs show that our approach achieves better and robust gains over the baseline and related NMT approaches. Our model further outperforms strong SMT baselines in some settings even without using ensembles.

==> tikz-qtree.tex <==
%    tikz-qtree.tex
%    Version 1.2, 20 Apr 2012

%    Copyright (C) 2002, 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.2:
% - level-specific styles (thanks to Andrew Stacey)

% New in version 1.11:
% - make options compatible with standard tikz trees

% New in version 1.1:
% - sideways trees

%% These macros facilitate building up an object recursively before
%% putting it into the input stream.

\newtoks\@result
\def\@call#1#2{\let\@cont=#2\bgroup\@result={}#1}
\def\@return{\global\@result=\@result\egroup\@cont}

\def\@ifequal#1#2{\edef\testa{#1}\edef\testb{#2}\ifx\testa\testb}

%% scan a tree: this just scans a subtree and then puts it onto the
%% input stream

\def\Tree{\@call\@subtree\@Tree}
\def\@Tree{%
%\showthe\@result %debug
\ifpgfpicture % is there a test for tikzpicture?
\pgftree{\the\@result}%
\else
\tikzpicture[baseline]\pgftree{\the\@result}\endtikzpicture
\fi
}

%% scan a subtree
\newtoks\child@list
\newtoks\root@node

\def\@subtree[{%
\root@node={}%
\pgfutil@ifnextchar.{\@call\@interior\@@subtree}{\@@@subtree}}
\def\@@subtree{%
\root@node=\@result
\@@@subtree
}
\def\@@@subtree{%
\@call\@children\@@@@subtree
}
\def\@@@@subtree]{%
\child@list=\@result
\pgfutil@ifnextchar.{\@call\@interior\@@@@@subtree}{\@@@@@@subtree}}
\def\@@@@@subtree{%
%%% Check for mismatch.
\@ifequal{\the\root@node}{\pgfutil@empty}%
  \root@node=\@result
\fi
\@ifequal{\the\root@node}{\the\@result}\else
  \message{Warning: mismatched labels, \the\root@node{} and \the\@result.}%
\fi
\@@@@@@subtree
}
\def\@@@@@@subtree{%
\@ifequal{\the\root@node}{\pgfutil@empty}%
\edef\act{\noexpand\@result={%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\noexpand\path coordinate (\noexpand\nodename);}{\the\child@list}}}%
\else
\edef\act{\noexpand\@result={%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\the\root@node}{\the\child@list}}}%
\fi
\act
\@return}

%% scan a sequence of subtrees or leaves

\newif\ifscanned@edge

\def\@children{%
\scanned@edgefalse
\child@list{}%
\@@children}
\def\@@children{%
\pgfutil@ifnextchar]{\@result\child@list\@return}{% end of children
\pgfutil@ifnextchar\edge{% explicit edge
\ifscanned@edge
\message{Warning: more than one edge given for a single child}\let\next\@@children % ignore
\else
\scanned@edgetrue\let\next\@@@children
\fi
\@call\@edge\next}{%
% else, a real node is next
\ifscanned@edge\else % no explicit edge, supply default
\expandafter\child@list\expandafter{\the\child@list{\edge@adapter{}}}%
\fi
\scanned@edgefalse
\pgfutil@ifnextchar[{% subtree
\expandafter\child@list\expandafter{\the\child@list{\level@hook\interior@hook}}%
\@call\@subtree\@@@children}%
{% leaf
\expandafter\child@list\expandafter{\the\child@list{\level@hook\frontier@hook}}%
\@call\@leaf\@@@children}%
}}}
\def\@@@children{%
% wrap child inside curly braces
\expandafter\@result\expandafter{\expandafter{\the\@result}}%
\edef\act{\noexpand\child@list{\the\child@list \the\@result}}\act
\@@children
}

\def\@interior.{\@result{\node[alias=\nodename][every tree node,every internal node,every level \the\pgftree@level\space node/.try]}\@label}

\def\@leaf{\@call\@label\@@leaf}
\def\@@leaf{\edef\act{\noexpand\@result{%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\noexpand\node[alias=\noexpand\nodename][every tree node,every leaf node,every level \noexpand\the\pgftree@level\space node/.try]\the\@result}{}}}\act\@return}

\def\@edge\edge #1;{%
\@result{\edge@adapter{#1}}%
\@return}
\def\edge@adapter#1{%
\let\tikzparentnode\parentnodename
\let\tikzchildnode\nodename
\path edge from parent #1;%
}

\def\level@hook{%
{\advance\pgftree@level by 1\relax
\xdef\@act{\noexpand\tikzset{level \the\pgftree@level/.try}}}\@act}
\def\subtree@hook{%
%\edef\act{\noexpand\tikzset{every tree node/.append code={\noexpand\tikzset{every level \the\pgftree@level+ node/.try}}}}\act
{\advance\pgftree@level by 1\relax
\xdef\@act{\noexpand\tikzset{level \the\pgftree@level+/.try}}}\@act
}
\def\interior@hook{\tikzset{interior/.try}}
\def\frontier@hook{\tikzset{frontier/.try}}

% a label is either text or PGF/TikZ code starting with \node
\def\@label{\pgfutil@ifnextchar\node{\@litlabel}{\@@label}}
\def\@@label#1 {%
\expandafter\@result\expandafter{\the\@result{#1};}%
\@return}

% try to copy \node command into \@result without stripping braces
\def\@litlabel\node{\@@litlabel}
\def\@@litlabel{\pgfutil@ifnextchar\bgroup{\@@@litlabel}{\@@@@litlabel}}
\def\@@@litlabel#1{\expandafter\@result\expandafter{\the\@result {#1}}\@@litlabel}
\def\@@@@litlabel#1;{\expandafter\@result\expandafter{\the\@result #1;}\@return}

% predefined edges

\def\tree@edge#1#2{(#1.\pgftree@parentanchor) -- (#2.\pgftree@childanchor)}

\def\roof@edge#1#2{\csname roof@edge@\leveldirection\endcsname{#1}{#2}}
\def\roof@edge@down#1#2{(#1.south) -- (#2.north west) -- (#2.north east) -- cycle}
\def\roof@edge@up#1#2{(#1.north) -- (#2.south west) -- (#2.south east) -- cycle}
\def\roof@edge@left#1#2{(#1.west) -- (#2.north east) -- (#2.south east) -- cycle}
\def\roof@edge@right#1#2{(#1.east) -- (#2.north west) -- (#2.south west) -- cycle}

%%% Options
\pgfkeysgetvalue{/tikz/level distance/.@cmd}{\orig@leveldistance}
\tikzoption{level distance}{\pgfmathsetlength\levelsep{#1}\orig@leveldistance#1\pgfeov}
\tikzoption{distance from root}{\pgfmathsetlength\levelsep{#1}\advance\levelsep by -\pgftree@depth}
\pgfkeysgetvalue{/tikz/sibling distance/.@cmd}{\orig@siblingdistance}
\tikzoption{sibling distance}{\pgfmathsetlength\subtreesep{#1}\orig@siblingdistance#1\pgfeov} % different semantics

% I don't really like this scheme
\pgfkeysgetvalue{/tikz/grow/.@cmd}{\orig@grow}
\tikzoption{grow}{\csname grow@#1\endcsname\orig@grow#1\pgfeov}
\pgfkeysgetvalue{/tikz/grow'/.@cmd}{\orig@growprime}
\tikzoption{grow'}{\csname growprime@#1\endcsname\orig@growprime#1\pgfeov}
\def\grow@up{\def\leveldirection{up}\def\siblingdirection{left}}
\def\grow@down{\def\leveldirection{down}\def\siblingdirection{right}}
\def\growprime@up{\def\leveldirection{up}\def\siblingdirection{right}}
\def\growprime@down{\def\leveldirection{down}\def\siblingdirection{left}}
\def\grow@left{\def\leveldirection{left}\def\siblingdirection{down}}
\def\grow@right{\def\leveldirection{right}\def\siblingdirection{up}}
\def\growprime@left{\def\leveldirection{left}\def\siblingdirection{up}}
\def\growprime@right{\def\leveldirection{right}\def\siblingdirection{down}}

% defaults appropriate for linguistic trees
\def\tikz@edge@to@parent@path{\tree@edge{\tikzparentnode}{\tikzchildnode}}
\tikzset{every tree node/.style={anchor=base}}
\tikzset{every leaf node/.style={}}
\tikzset{every internal node/.style={}}

% predefined roof style
\tikzset{roof/.style={edge from parent path=\roof@edge{\tikzparentnode}{\tikzchildnode}}}

